CORTEX-AVD: A Framework for CORner Case Testing and EXploration in Autonomous Vehicle Development

Autonomous Vehicles (AVs) aim to improve traffic safety and efficiency by reducing human error. However, ensuring AVs reliability and safety is a challenging task when rare, high-risk traffic scenarios are considered. These 'Corner Cases' (CC) scenarios, such as unexpected vehicle maneuvers or sudden pedestrian crossings, must be safely and reliable dealt by AVs during their operations. But they arehard to be efficiently generated. Traditional CC generation relies on costly and risky real-world data acquisition, limiting scalability, and slowing research and development progress. Simulation-based techniques also face challenges, as modeling diverse scenarios and capturing all possible CCs is complex and time-consuming. To address these limitations in CC generation, this research introduces CORTEX-AVD, CORner Case Testing & EXploration for Autonomous Vehicles Development, an open-source framework that integrates the CARLA Simulator and Scenic to automatically generate CC from textual descriptions, increasing the diversity and automation of scenario modeling. Genetic Algorithms (GA) are used to optimize the scenario parameters in six case study scenarios, increasing the occurrence of high-risk events. Unlike previous methods, CORTEX-AVD incorporates a multi-factor fitness function that considers variables such as distance, time, speed, and collision likelihood. Additionally, the study provides a benchmark for comparing GA-based CC generation methods, contributing to a more standardized evaluation of synthetic data generation and scenario assessment. Experimental results demonstrate that the CORTEX-AVD framework significantly increases CC incidence while reducing the proportion of wasted simulations.

==> Tabs/SCENIC_VARIABLES.tex <==
\setlength{\tabcolsep}{1pt}
% \begin{table*}[h]
\begin{table}[h]
\caption{Scenic parameters - \textcolor{red}{ACHO QUE A COLUNA DE TIPO NÃO FAZ SENTIDO. É TUDO FLOAT. APAGAR}}
\label{tab:scenic_variables}
\centering
% \begin{tabularx}{\textwidth}{|m{2.5cm}|m{9cm}|m{5cm}|}
% \begin{tabularx}{\textwidth}{|m{2.5cm}|m{2.8cm}|m{2.8cm}|}
% \begin{tabularx}{\textwidth}{|x|x|x|}
\begin{tabular}{@{}lcl@{}}
 % \toprule
 \cmidrule(){1-3}
 \textbf{Parameters} & \textbf{Type} & \textbf{Interval} \\ 
 % \hline
 \cmidrule(){1-3}
 \scriptsize{EGO\_INIT\_DIST} & \textit{numeric} & \scriptsize{{[}0, +$\infty${[}} \\
 % \hline
 \cmidrule(){1-3}
 \scriptsize{EGO\_SPEED}      & \textit{numeric} & \scriptsize{{[}5, 80{]}} \\
 % \hline
 \cmidrule(){1-3}
 \scriptsize{EGO\_BRAKE}      & \textit{float}   & \scriptsize{{[}0, 1{]}} \\
 % \hline
 \cmidrule(){1-3}
 \scriptsize{ADV\_INIT\_DIST} & \textit{numeric} & \scriptsize{{[}0, +$\infty${[}} \\
 % \hline
 \cmidrule(){1-3}
 \scriptsize{ADV\_SPEED}      & \textit{float}   & \scriptsize{{[}5, 80{]}} \\
 % \hline
 \cmidrule(){1-3}
 \scriptsize{SAFETY\_DIST}    & \textit{float}   & \scriptsize{{[}0, 20{]}} \\
 % \hline
 \cmidrule(){1-3}
 \scriptsize{CRASH\_DIST}     & \textit{float}   & \scriptsize{{[}0, 5{]}} \\
 % \hline
 \cmidrule(){1-3}
% \end{tabularx}
\end{tabular}
% \end{table*}
\end{table}

